Periodic thermodynamics of isolated systems

The nature of the behaviour of an isolated many-body quantum system periodically driven in time has been an open question since the beginning of quantum mechanics. After an initial transient, such a system is known to synchronize with the driving; in contrast to the non-driven case, no fundamental principle has been proposed for constructing the resulting non-equilibrium state. Here, we analytically show that, for a class of integrable systems, the relevant ensemble is constructed by maximizing an appropriately defined entropy subject to constraints, which we explicitly identify. This result constitutes a generalisation of the concepts of equilibrium statistical mechanics to a class of far-from-equilibrium-systems, up to now mainly accessible using ad-hoc methods.

==> macros.tex <==
\newcommand{\bra}[1]{\left< #1 \right|}
\newcommand{\ket}[1]{\left| #1 \right>}
\newcommand{\heff}{\hat{H}_{\mathrm{eff}}}
\newcommand{\tred}[1]{{\color{red} {#1}}}
\newcommand{\tblue}[1]{{\color{blue} #1}}
\newcommand{\eps}{\epsilon}
\newcommand{\mI}[1]{\hat{\mathcal{I}}_{#1}}
\newcommand{\U}[2]{\hat{U}(#1,#2)}
\newcommand{\Ud}[2]{\hat{U}^\dagger(#1,#2)}
\newcommand{\mA}{\hat{\mathcal{A}}}
\newcommand{\tc}{\tilde{a}}
\newcommand{\tb}{\tilde{b}}
\newcommand{\hb}{\hat{b}}
\newcommand{\hbd}{\hat{b}^\dagger}
\newcommand{\hc}{\hat{c}}
\newcommand{\ha}{\hat{a}}
\newcommand{\hcd}{\hat{c}^\dagger}
\newcommand{\hh}{\hat H}
\newcommand{\mb}{}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\hs}{\hat{\sigma}}

